ED-Copilot: Reduce Emergency Department Wait Time with Language Model Diagnostic Assistance

In the emergency department (ED), patients undergo triage and multiple laboratory tests before diagnosis. This time-consuming process causes ED crowding which impacts patient mortality, medical errors, staff burnout, etc. This work proposes (time) cost-effective diagnostic assistance that leverages artificial intelligence systems to help ED clinicians make efficient and accurate diagnoses. In collaboration with ED clinicians, we use public patient data to curate MIMIC-ED-Assist, a benchmark for AI systems to suggest laboratory tests that minimize wait time while accurately predicting critical outcomes such as death. With MIMIC-ED-Assist, we develop ED-Copilot which sequentially suggests patient-specific laboratory tests and makes diagnostic predictions. ED-Copilot employs a pre-trained bio-medical language model to encode patient information and uses reinforcement learning to minimize ED wait time and maximize prediction accuracy. On MIMIC-ED-Assist, ED-Copilot improves prediction accuracy over baselines while halving average wait time from four hours to two hours. ED-Copilot can also effectively personalize treatment recommendations based on patient severity, further highlighting its potential as a diagnostic assistant. Since MIMIC-ED-Assist is a retrospective benchmark, ED-Copilot is restricted to recommend only observed tests. We show ED-Copilot achieves competitive performance without this restriction as the maximum allowed time increases. Our code is available at https://github.com/cxcscmu/ED-Copilot.

==> Tables/backbone.tex <==

% \begin{table}
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%         Backbone & F1 & AUC  & Cost \\
%     \hline
%         Biogpt (347m)& 0.403 & 0.807 & 265 \\
%     \hline
%         Pythia (70m) & 0.397 & 0.813 & 265\\
%     \hline
%         Gpt2-medium (345m)& 0.401 & 0.808 & 265 \\
%     \hline
%         Biogpt (347m)& 0.397 & 0.790 & 134 \\
%     \hline
%         Pythia (70m) & 0.290 & 0.698 & 166 \\
%     \hline
%         Gpt2-medium (345m)& 0.358 & 0.757  &133 \\
%     \hline
%     \end{tabular}
%     \caption{Performance of different backbone on Critical Outcome}
%     \label{backbone}
% \end{table}
\begin{table}
    \caption{Performance of different backbone on Critical Outcome}
    \label{backbone}
    \centering
    \begin{tabular}{l|c|c|c}
    \hline
       Model & F1 & AUC & Cost \\
    \hline
        Biogpt (347m)& 0.413 & 0.820 & 125 \\
    \hline
        Pythia (70m) & 0.290 & 0.698 & 166 \\
    \hline
        Gpt2-medium (345m)& 0.358 & 0.757  &133 \\
    \hline
    \end{tabular}
\end{table}

\by{In Table 9, pls add the default PLM results and order the rows according to performance?}

==> Tables/importance.tex <==

\begin{table}[h]
    \caption{Feature Importance on Critical Outcome}
    \label{importance}
    \centering
    \begin{tabular}{l|c|c}
    \hline
         Model & F1 & AUC  \\
    \hline
         ED-Copilot(Full feature) & 0.413 & 0.820   \\
    \hline
         w/o. triage& 0.277 & 0.704  \\
    \hline
         w/o. CBC& 0.385 & 0.803  \\
    \hline
         w/o. Chem& 0.420 & 0.827   \\
    \hline
    \end{tabular}
\end{table}

==> Tables/linearization.tex <==

\begin{table}
    \caption{Linearization with dummy name}
    \label{linearization}
    \centering

\resizebox{\textwidth/2}{!}{
    \begin{tabular}{l|c|c|c|c|c|c}
    \hline
    & \multicolumn{3}{c|}{Critical outcome} & \multicolumn{3}{c}{ED LOS} \\
    \cline{2-7}
    Linearization Technique & F1 & AUC & Cost & F1 & AUC & Cost \\
    \hline
    True Name & 0.397 & 0.777 & 134 & 0.241 & 0.695 & 144  \\
    \hline
    Dummy Name & 0.413 & 0.820 & 125 & 0.252 & 0.707 & 154  \\
    \hline
    \end{tabular}
}
\end{table}

==> Tables/llama.tex <==

\begin{table*}[h]
  \centering

\caption{Results with additional LLM baselines}

\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\hline
\multirow{2}{*}{\textbf{Model}}& \multicolumn{5}{c}{\textbf{Critical Outcome}}                            & \multicolumn{5}{c}{\textbf{Lengthened ED Stay}}                            \\ \cline{2-11} 
\multicolumn{1}{c}{}                        & F1     & AUC   & Sensitivity & Specificity & Avg Test Time & F1     & AUC   & Sensitivity & Specificity & Avg Test Time \\ \hline
BioGPT without RL                             & 0.381  & 0.810 & 0.725       & 0.765       & 265           & 0.236  & 0.718 & 0.710       & 0.620       & 265           \\ \hline
Llama 7B (lora) without RL                    & 0.397  & 0.798 & 0.692       & 0.767       & 265           & 0.232  & 0.701 & 0.705       & 0.610       & 265           \\ \hline
 ED Co-pilot (BioGPT with RL)                             & 0.413  & 0.820 & 0.750       & 0.779       & 125           & 0.252  & 0.707 & 0.725       & 0.606       & 154           \\ \hline
\end{tabular}%
}
  \label{tab:llama}
\end{table*}



==> Tables/personalization2.tex <==




% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c}
%         \hline
%                 & F1    & AUC \\
%         \hline
%          Random Forest (2 groups)& 0.267& 0.790 \\
%         \hline
%          XGBoost(2 groups)& 0.312 & 0.789\\
%         \hline
%          LightGBM(2 groups)& 0.352 & 0.795 \\
%         \hline
%          ED-Copilot& 0.398 & 0.820 \\
%          \hline
%     \end{tabular}
%     \caption{Group 1 by number of labs}
%     \label{group1}
% \end{table}

% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c}
%         \hline
%                 & F1    & AUC \\
%         \hline
%          Random Forest(2 groups)& 0.332 & 0.797 \\
%         \hline
%          XGBoost(2 groups)& 0.360 & 0.777\\
%         \hline
%          LightGBM(2 groups)& 0.389 & 0.797 \\
%         \hline
%          ED-Copilot& 0.416& 0.777\\
%         \hline
%     \end{tabular}
%     \caption{Group 2 by number of labs}
%     \label{group2}
% \end{table}

% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c}
%         \hline
%                 & F1    & AUC \\
%         \hline
%          Random Forest(2 groups)& 0.50 & 0.784 \\
%         \hline
%          XGBoost(2 groups)& 0.603 & 0.796\\
%         \hline
%          LightGBM(2 groups)& 0.618 & 0.796 \\
%         \hline
%          ED-Copilot& 0.551 & 0.781 \\
%         \hline
%     \end{tabular}
%     \caption{Group 3 by number of labs}
%     \label{group3}
% \end{table}



% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c}
%         \hline
%             ED-Copilot    & F1    & AUC \\
%         \hline
%          Group 1& 0.398 & 0.820 \\
%         \hline
%          Group 2& 0.416 & 0.777\\
%         \hline
%          Group 3& 0.551 & 0.781 \\
%         \hline
%     \end{tabular}
%     \caption{Group by number of lab groups per patient}
%     \label{personalization2}
% \end{table}

\begin{table*}[h]
\caption{Personalization Results based on the number of lab groups}
\label{major}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Top} (109/1334)} & \multicolumn{3}{c}{\textbf{Medium} (174/1334)} & \multicolumn{3}{c}{\textbf{Rare}(26/60)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
\textbf{Model} & F1 & Sensitivity & Specificity & F1 & Sensitivity & Specificity & F1 & Sensitivity & Specificity \\
\midrule
Random Forest (Top 2 groups) & 0.267 & 0.716 & 0.731 & 0.332 & 0.736 & 0.750 & 0.500 & 0.846 & 0.667 \\
XGBoost (Top 2 groups) & 0.312 & 0.789 & 0.694 & 0.360 & 0.770 & 0.669 & 0.603 & 0.692 & 0.733 \\
LightGBM (Top 2 groups) & 0.352 & 0.761 & 0.724 & 0.389 & 0.799 & 0.683 & 0.618 & 0.654 & 0.883 \\
ED-Copilot (Personalized) & 0.398 & 0.737 & 0.771 & 0.416 & 0.740 & 0.739 & 0.551 & 0.7 & 0.729 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Tables/suggestion.tex <==

\begin{table}
    \caption{Lab group suggestion \cx{maybe a figure}}
    \label{suggestion}
    \centering
    \resizebox{\textwidth/2}{!}{
    \begin{tabular}{l|c|c|c|c}
    \hline
         & Micro F1 & Macro F1  & Weighted F1  & BLUE-1\\
    \hline
        Critical Outcome & 0.7713  & 0.628 & 0.758  & \\
    \hline
        ED LOS &  &  &  & \\
    \hline
    \end{tabular}}
\end{table}

==> Tables/triage.tex <==

\begin{table*}[h]
    \caption{Triage}
    \centering
    \begin{tabular}{|c|}
    \hline
        Temperature\\
    \hline
        Heart rate\\
    \hline
        Respiratory rate\\
    \hline
        Oxygen saturation\\
    \hline
        Systolic blood pressure\\
    \hline
        Diastolic blood pressure\\
    \hline
        Self-reported pain\\
    \hline
        Emergency severity index acuity\\
    \hline
        Chief complaint\\
    \hline
    \end{tabular}
    \label{triage}
\end{table*}

==> Tables/uncertainty.tex <==

\begin{table*}[h]
  \centering

\caption{Major Results with uncertainty quantification}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Critical Outcome}}                              & \multicolumn{5}{c}{\textbf{Lengthened ED Stay}}                             \\ \cline{2-11} 
                       & F1             & AUC           & Sensitivity     & Specificity     & Avg Test Time & F1             & AUC           & Sensitivity     & Specificity     & Avg Test Time \\ \hline
Random Forest          & 0.377 (0.015)  & 0.807 (0.011) & 0.754 (0.012)   & 0.748 (0.005)   & 265           & 0.206 (0.014)  & 0.698 (0.011) & 0.693 (0.016)   & 0.616 (0.024)   & 265           \\ 
XGBoost                & 0.379 (0.019)  & 0.807 (0.009) & 0.731 (0.017)   & 0.744 (0.006)   & 265           & 0.212 (0.010)  & 0.679 (0.007) & 0.619 (0.020)   & 0.661 (0.020)   & 265           \\ 
LightGBM               & 0.394 (0.016)  & 0.813 (0.008) & 0.725 (0.012)   & 0.769 (0.004)   & 265           & 0.217 (0.015)  & 0.705 (0.011) & 0.706 (0.017)   & 0.605 (0.014)   & 265           \\ 
3-layer DNN            & 0.339 (0.032)  & 0.743 (0.021) & 0.676 (0.024)   & 0.683 (0.011)   & 265           & 0.194 (0.031)  & 0.637 (0.013) & 0.649 (0.015)   & 0.593 (0.014)   & 265           \\ \hline
SM-DDPO                & 0.353 (0.031)  & 0.780 (0.020) & 0.685 (0.023)   & 0.763 (0.022)   & 182 (32)      & 0.183 (0.028)  & 0.619 (0.012) & 0.472 (0.012)   & 0.739 (0.011)   & 177 (60)      \\ 
ED-Copilot             & 0.413 (0.028)  & 0.820 (0.021) & 0.750 (0.018)   & 0.779 (0.011)   & 125 (21)      & 0.232 (0.023)  & 0.707 (0.015) & 0.725 (0.018)   & 0.606 (0.015)   & 154 (33)      \\ \hline
\end{tabular}%
}
  \label{tab:uncertainty}
\end{table*}


